Efficient Approximate Query Answering over Sensor Data with Deterministic Error Guarantees

With the recent proliferation of sensor data, there is an increasing need for the efficient evaluation of analytical queries over multiple sensor datasets. The magnitude of such datasets makes exact query answering infeasible, leading researchers into the development of approximate query answering approaches. However, existing approximate query answering algorithms are not suited for the efficient processing of queries over sensor data, as they exhibit at least one of the following shortcomings: (a) They do not provide deterministic error guarantees, resorting to weaker probabilistic error guarantees that are in many cases not acceptable, (b) they allow queries only over a single dataset, thus not supporting the multitude of queries over multiple datasets that appear in practice, such as correlation or cross-correlation and (c) they support relational data in general and thus miss speedup opportunities created by the special nature of sensor data, which are not random but follow a typically smooth underlying phenomenon. To address these problems, we propose PlatoDB; a system that exploits the nature of sensor data to compress them and provide efficient processing of queries over multiple sensor datasets, while providing deterministic error guarantees. PlatoDB achieves the above through a novel architecture that (a) at data import time pre-processes each dataset, creating for it an intermediate hierarchical data structure that provides a hierarchy of summarizations of the dataset together with appropriate error measures and (b) at query processing time leverages the pre-computed data structures to compute an approximate answer and deterministic error guarantees for ad hoc queries even when these combine multiple datasets.

==> 1.Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
%sensor data is big
In the era of  Internet of Things (IoT), sensor devices are equipped everywhere to serve many different monitoring applications including air quality monitoring, urban energy controlling, and public health caring. Data comes from these devices typically has high granularity and requires substantial storage ranging from a few GB to many TB~\cite{LeeBWSTLYGG13,KalakantiSRM15}. For instance, a Formula 1 race car produces 20GB of data during two 90-minute practice sessions~\footnote{http://www.zdnet.com/article/formula-1-racing-sensors-data-speed-and-the-internet-of-things/}, while a commercial aircraft may generate 2.5TB of data per day~\footnote{http://www.datasciencecentral.com/profiles/blogs/that-s-data-science-airbus-puts-10-000-sensors-in-every-single}.

% OLAP queries are important, but inefficient
There is an increasing demand to issue OLAP (Online Analytical Processing) queries over different sensor data (also called time series data) in order to explore the underlying relationships. For example, computing the correlation of the temperature sensor data and the number of entrance sensor data can help making a good energy saving plan. However, running OLAP queries over the big sensor data can be very expensive, as the queries have to access significant amounts of data. This problem becomes worse when queries combine multiple sensor datasets. For example, it takes more than 12 minutes to compute the correlation between two sensor data with 10 billion data points. To improve the performance, there are two typical strategies: (i) using expensive computing infrastructures, i.e.,  use distributed processing systems such as Hadoop and Spark to scale up their computing infrastructures; and (ii) returning approximate answers instead of accurate answers. In this work, we follow the second strategy.

% existing work. Sampling and compression
There have been works on approximating the result of queries through a variety of techniques~\cite{AgarwalMPMMS13,acharya2000congressional,babcock2003dynamic,rosch2009sample}, which can be classified into two categories: (i) sampling-based methods, and (ii) compression-based approaches. Sampling-based methods (e.g., BlinkDB~\cite{AgarwalMPMMS13}) first choose a subset of the data to execute the queries, then scale up the answer by a factor of the original data size over the sampling size. Compression-based approaches uses a function (e.g., Piecewise Aggregate Approximation (PAA) ~\cite{KeoghCPM01} and  the Piecewise Linear Representation (PLR)~\cite{keogh1997fast}) to represent a sensor data segment, then run the queries directly on the data driven by the functions instead of the original data. Though they can efficiently return approximate answers, there are no absolute error guarantees, i.e., the errors between approximate answers and accurate answers are not bounded deterministically.


%our method
To overcome the limitations, we design a system called \emph{\db}, which allows users to pose OLAP queries (formally defined in Section~\ref{sec:DataQueries}) along with error bound constraints (also called error budgets) and returns approximate answers efficiently with errors no greater than the given error bound constraints~\footnote{\db{} also supports OLAP queries along with response time constraints.}. More precisely, \db\ operates as follows: When it is initiated, it preprocesses each sensor data individually and builds a hierarchical tree structure for each dataset (Section~\ref{sec:index}). A node in the tree structure refers to one segment of sensor data (i.e., a subsequence of the original sensor data) and includes two components: (i) \textit{a compression function} representing the segment, e.g., PAA~\cite{KeoghCPM01} uses a constant function while PLR~\cite{keogh1997fast} uses a one degree polynomial function, and (ii) \textit{error measures} capturing the statistics of the segment and also the difference between the original data and the compressed data. During runtime, \db{}  takes as input an OLAP query over multiple sensor datasets together with an error budget and accesses the corresponding tree structures in a top-down way (Section~\ref{sec:QueryProcessing}). In each step, \db{} greedily jumps from a node to its children nodes to maximize the error reduction. It finally output an approximate answer annotated with an error no greater than the error budget.





\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{Figure/architecture_combined.pdf}
\caption{\db's architecture, including details on the \tree\ generation and query processing.}
\label{fig:architecture}
\end{figure*}

\smallskip

\noindent\textbf{Contributions.}
To summarize, this paper makes the following contributions:

\begin{itemize}
  \item We formally define a query language, which is powerful enough to express most common statistic queries, e.g., variance, correlation, and cross-correlation (Section~\ref{sec:DataQueries}).
  \item We develop an error estimation method to estimate error for any given queries. More precisely, we store extra error measures for each compressed sensor data segment and use the error measures to estimate errors (Section~\ref{Sec:error_estimator}).
  \item We propose two algorithms, i.e., top-down algorithm and bottom-up algorithm, to build a novel \tree\ structure for each sensor data, which is able to provide different levels of error guarantees (Section~\ref{sec:index}).
  \item We propose a greedy query processing algorithm running on the \tree s. We theoretically prove that there is no optimal algorithm that can always access minimal number of nodes. However, we prove that if the \tree s satisfy a certain condition, the greedy algorithm is optimal. (Section~\ref{sec:QueryProcessing}).
  \item We conduct experiments on two real-life datasets to evaluate our algorithms. The results show that our algorithm outperforms the baselines by 1-3 orders of magnitudes (Section~\ref{experiments}).
\end{itemize}

%\begin{itemize}
%\item We propose a theoretical analysis on how to generate signatures for each segment of a data that can provide error guarantees. The signatures can handle any polynomial estimation functions.
%\item We build a novel \tree\ structure to organize signatures for each data. The tree structure provides different levels of error guarantees.
%\item We design an efficient query processing algorithm operating on tree structures. In addition, we theoretically prove its optimality property.
%\item We conduct experiments on four real-life datasets to evaluate our algorithms. The results show that our algorithm outperforms the baselines by up to one order of magnitude.
%\end{itemize}







